Coswara: A website application enabling COVID-19 screening by analysing respiratory sound samples and health symptoms

The COVID-19 pandemic has accelerated research on design of alternative, quick and effective COVID-19 diagnosis approaches. In this paper, we describe the Coswara tool, a website application designed to enable COVID-19 detection by analysing respiratory sound samples and health symptoms. A user using this service can log into a website using any device connected to the internet, provide there current health symptom information and record few sound sampled corresponding to breathing, cough, and speech. Within a minute of analysis of this information on a cloud server the website tool will output a COVID-19 probability score to the user. As the COVID-19 pandemic continues to demand massive and scalable population level testing, we hypothesize that the proposed tool provides a potential solution towards this.

==> table_old_sound_categories.tex <==
\begin{table*}[]
\rowcolors{2}{white}{gray!10}
\begin{tabular}{p{2.5cm}|p{13.5cm}}
\hline
\rowcolor[HTML]{9B9B9B} 
\textbf{Stimulus} & \textbf{Remarks} \\ \hline
breathing deep, breathing shallow         &  Breathing sound involves respiratory tract, lungs etc. It may contain COVID-19 bio-marker as it affects lungs. Breathing deep is produced by more respiratory effort.\\ \hline
cough heavy, cough shallow          & Cough production uses respiratory tract, glottis, lungs etc. It may contain COVID-19 bio-marker if it is present in voicebox. Coughing heavily requires more involvement of lower respiratory organs.\\ \hline
    vowel a, vowel e and vowel o        &  These are sustained phonation of three different vowels. They involve vocal tract, tongue, oral cavity etc. They may contain COVID-19 bio-marker if it has effect on vowel formant frequencies. \\ \hline
    counting fast and counting normal            & It is the counting of digits from 1 to 20. Complete voice production and associated system is involved in this sound. It may contain COVID-19 signature that is not captured in above categories because speech is more complicated sound\\ \hline
\end{tabular}
\caption{Stimulus categories and their significance}
\label{resp_table}
\end{table*}

==> table_subject_categories.tex <==
\begin{table}[]
\centering
\rowcolors{2}{white}{gray!10}
\resizebox{\columnwidth}{!}
{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Subject Category} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{Description}} \\ \midrule
Non-COVID &  & Not infected with COVID-19 \\
COVID-Pre-O &  & \begin{tabular}[c]{@{}l@{}}Infected with COVID-19 with\\ a strain earlier to Omicron outbreak\end{tabular} \\
COVID-O &  & \begin{tabular}[c]{@{}l@{}}Infected with COVID-19 with\\ a strain during Omicron outbreak\end{tabular} \\ \bottomrule
\end{tabular}
}
\caption{}
\label{tab:my-table}
\end{table}

==> table_subject_sound_categories.tex <==
% \begin{table}[]
% \centering
% \rowcolors{2}{white}{gray!10}
% \resizebox{\columnwidth}{!}
% {
% \begin{tabular}{@{}lll@{}}
% \toprule
% \textbf{Sound Category} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{Description}} \\ \midrule
% Breathing-shallow/deep &  & \begin{tabular}[c]{@{}l@{}}Few cycles of inspiration and expiration:\\ without (shallow)/with (deep) exertion on the lungs\end{tabular} \\
% Cough-shallow/heavy &  & \begin{tabular}[c]{@{}l@{}}Few bouts of cough:\\ without (shallow)/with (heavy) exertion on the lungs\end{tabular} \\
% Vowel-[u]/[i]/[\ae] &  & \begin{tabular}[c]{@{}l@{}}Sustained phonation of three different vowels:\\ $[$u] as in boot, [i] as in beet, and [\ae] as in bat\end{tabular} \\
% Counting-normal/fast &  & \begin{tabular}[c]{@{}l@{}}Counting numbers from 1 to 20 in:\\ normal/fast pace\end{tabular} \\ \bottomrule
% \end{tabular}
% }
% \caption{}
% \label{tab:my-table}
% \end{table}


\begin{table}[]
\centering
\rowcolors{2}{white}{gray!10}
% \resizebox{\columnwidth}{2.75cm}
{
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Subject Category} &   \multicolumn{1}{c}{\textbf{Description}} \\ \midrule
Healthy ($H$) &   \begin{tabular}[c]{@{}l@{}}Healthy subjects, not infected with\\ SARS-CoV-2\end{tabular}  \\
Delta ($Del$) &   \begin{tabular}[c]{@{}l@{}}Infected with SARS-CoV-2 with\\ a strain earlier to Omicron outbreak\end{tabular} \\
Omicron ($Omi$) &  \begin{tabular}[c]{@{}l@{}}Infected with SARS-CoV-2 with\\ a strain during Omicron outbreak\end{tabular} \\
Positive ($Pos$) &  \begin{tabular}[c]{@{}l@{}}Del and Omi subjects pooled\end{tabular} \\\midrule
\multicolumn{1}{c}{\textbf{Sound Category}} &  \multicolumn{1}{c}{\textbf{Description}} \\ \midrule
Breathing-shallow/deep &  \begin{tabular}[c]{@{}l@{}}Few cycles of inspiration/expiration:\\ with shallow/deep exertion on lungs\end{tabular} \\
Cough-shallow/heavy &   \begin{tabular}[c]{@{}l@{}}Few bouts of cough:\\ with shallow/heavy exertion on   lungs\end{tabular} \\
Vowel-[u]/[i]/[\ae] &   \begin{tabular}[c]{@{}l@{}}Sustained phonation of three vowels:\\ $[$u] in boot, [i] in beet, [\ae] in bat\end{tabular} \\
Counting-normal/fast &  \begin{tabular}[c]{@{}l@{}}Counting numbers from $1$ to $20$ at:\\ normal/fast pace\end{tabular} \\ \bottomrule
\end{tabular}
}
%\vspace{0.1in}
\caption{Subject and sound categories analyzed in this study}
\vspace{-0.35in} 
\label{tab:subject_sound_categroies}
\end{table}

==> test_auc.tex <==
\begin{table*}[]
\rowcolors{2}{white}{gray!10}
\begin{tabular}{p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1cm}p{1cm}p{0.8cm}p{0.8cm}p{0.8cm}p{2cm}}
\hline
% \rowcolor[HTML]{9B9B9B} 
\textbf{Task} & \bf Breathing-deep &\bf Breathing-shallow & \bf Cough-heavy & \bf Cough-shallow & \bf Counting-fast  & \bf Counting-normal & \bf Vowel-[\ae] & \bf Vowel-[e] & \bf Vowel-[o] & \bf Fusion (Sensitivity at 95\% Specificity)\\ \hline
    \textbf{Omi-Del}      &       79.9      &     73.4        & 65.2  &   65.7  & 81.4  &  79.8 &  73.0 & 75.3  &  77.9 &  89.0 (52.4)   \\ \hline
    \textbf{Del-H}       &      73.3       &     70.1        & 72.2  &  75.0   & 81.3   & 80.5  & 70.9  & 70.3  & 71.1 & 88.3 (68.6)\\ \hline
     \textbf{Omi-H}      &     80.2        &     76.9        & 81.2  &   83.7  &  84.0 & 82.1  & 75.8  & 79.5  & 74.9  & 93.1 (71.4) \\ \hline
     \textbf{Pos-H}       &      76.1       &    74.4         & 76.7  &  80.1   & 83.4  & 82.0  & 75.4  & 76.6  &  75.0 & 90.5 (71.4) \\ \hline
\end{tabular}
\caption{Depiction of AUC for different classification tasks on the held out test set.}
\label{test_auc_table}
\vspace{-0.3in} 
\end{table*}

% \begin{table*}[]
% \rowcolors{2}{white}{gray!10}
% \begin{tabular}{p{2.5cm}p{1cm}p{1cm}p{1cm}p{1cm}}
% \hline
% \rowcolor[HTML]{9B9B9B} 
% \textbf{Sound Category} & \textbf{O vs D} & \textbf{D vs H} & \textbf{O vs H} & \textbf{P vs H}\\ \hline
% breathing-deep          &             &             &   &          \\ \hline
% breathing-shallow       &            &            &  &          \\ \hline
% cough-heavy             &             &            &    &         \\ \hline
% Cough-shallow           &             &             &  &           \\ \hline
% counting-fast           &             &            &    &         \\ \hline
% counting-normal         &             &             &   &          \\ \hline
% vowel-a                 &             &            &   &          \\ \hline
% vowel-e                 &           &            &   &          \\ \hline
% vowel-o                 &             &            &    &         \\ \hline
% \end{tabular}
% \caption{Table of test AUCs}
% \label{val_auc_table}
% \end{table*}
